Individually Stable Dynamics in Coalition Formation over Graphs

Coalition formation over graphs is a well studied class of games whose players are vertices and feasible coalitions must be connected subgraphs. In this setting, the existence and computation of equilibria, under various notions of stability, has attracted a lot of attention. However, the natural process by which players, starting from any feasible state, strive to reach an equilibrium after a series of unilateral improving deviations, has been less studied. We investigate the convergence of dynamics towards individually stable outcomes under the following perspective: what are the most general classes of preferences and graph topologies guaranteeing convergence? To this aim, on the one hand, we cover a hierarchy of preferences, ranging from the most general to a subcase of additively separable preferences, including individually rational and monotone cases. On the other hand, given that convergence may fail in graphs admitting a cycle even in our most restrictive preference class, we analyze acyclic graph topologies such as trees, paths, and stars.

==> monotonic_short.tex <==
Before starting, let us note that individual stability and Nash stability are equivalent when the instance is monotone, since no player refuses that another enters her coalition.

We shall prove that, under monotone preferences, the IS dynamics always converge on paths.
Roughly speaking, the proof assumes that a cycle exists in the dynamics and exhibits a contradiction as follows. Consider any player $i$, being the rightmost of coalition $C$, joining in the dynamics the coalition $C'$ on her right. We prove that, in order for player $i$ to go back to her original coalition $C$, the rightmost player in $C'$, say player $i'$, has to join coalition $C''$, being on the right of $i'$. By iteratively repeating this argument, we obtain that the rightmost player of the path should also join the coalition on her right: a contradiction, given that no coalition exists on her right.
It is therefore possible to prove the following theorem.

\begin{theorem}\label{thm:paths:monotone} 
Under monotone preferences, the IS dynamics always converge on paths.
\end{theorem}





==> proof-thm-trees.tex <==
 We start with some notation. 
 We denote by $N(i)$ the set of neighbours of $i$  (we assume $i \notin N(i)$) and by $L(i)$ the set of edges incident to $i$.
For every feasible partition $\pi$ we define $L_{\pi} = \{(i,j) \in L : \pi(i) = \pi(j)\}$ and $\overline{L}_{\pi} = L\setminus L_{\pi}$ and we refer to them as the set of \emph{built} and \emph{broken} edges in $\pi$, respectively.
For every player $i$ and feasible partition $\pi$ we define $L_{\pi}(i) = \{(i,j): (i,j) \in L(i) \cap  L_{\pi}\}$  and $\overline{L}_{\pi}(i) = L(i)\setminus L_{\pi}(i)$, that are the set of built and broken edges incident to $i$, and we denote by $u_i(\pi)$ the utility of $i$ in $\pi$. 


The fact that $(N, L)$ is a tree directly implies that every feasible partition $\pi$ satisfies the  following  property.  
\begin{claim}\label{tree:claim1}
%Let $\pi$ be any feasible partition. For every pair of edges $(i,j), (i,j') \in \overline{L}_{\pi}(i)$ with $j\neq j'$, we have $\pi(j) \neq \pi(j')$.
Let $\pi$ be any feasible partition.
Given  any $i\in N$ then, for every $j, j'  \in N(i)$ such that  $j'\neq j$ and $(i,j) \in \overline{L}_{\pi}(i)$, it holds that $\pi(j) \neq \pi(j')$. 
%Given any $j$ such that $(i,j) \in \overline{L}_{\pi}(i)$, for any $j' \neq j$, $j' \in N(i)$, it holds that $\pi(j) \neq \pi(j')$.
\end{claim}

%\commentLuca{Maybe a slightly stronger version of Claim is needed: Let $\pi$ be any feasible partition. Given any $j$ such that $(i,j) \in \overline{L}_{\pi}(i)$, for any $j' \neq j$, $j' \in N(i)$, it holds that $\pi(j) \neq \pi(j')$.}



The deviation of a player $i$ in a feasible partition $\pi$ can be interpreted as selecting a neighboring  vertex $j$ that is incident to an edge in $\overline{L}_{\pi}(i)$.  
This observation enables us to describe  IS dynamics  
in a tree, as outlined in Algorithm \ref{alg:is:tree}. 
In order to prove the theorem, we incorporate a labeling scheme $\ell$, where $\ell: L \rightarrow N \cup \{\bot\}$ is a function labelling the edges of the graph as specified in Algorithm \ref{alg:is:tree}.



 \begin{algorithm}                      
\caption{IS dynamics for trees with labelling}         
\label{alg:is:tree}                          
\begin{algorithmic}[1]                  
\REQUIRE a graph hedonic game $(N,(\succeq_i)_{i\in N},L)$, such that $(N, L)$ is a tree, and an initial feasible partition $\pi^0$
\ENSURE A feasible partition $\pi$ of $N$ 
\STATE $t \gets 0$
\FOR{each $e \in L$}
\STATE ${\ell^{t}}(e) \gets \bot$ \label{alg:tree:label-init}
\ENDFOR
\WHILE{there exists $(\alpha^t, \beta^t) \in \overline{L}_{\pi^{t}}(\alpha^t)$ 
such that $\alpha^t$ has an IS deviation from $\pi^{t}(\alpha^t)$ to $\pi^{t}(\beta^{t})$
%such that the deviation of $\alpha^t$ from $\pi^{t}(\alpha^t)$ to $\pi^{t}(\beta^{t})$ is feasible
%\commentLuca{such that $\alpha^t$ has an IS deviation from $\pi^{t}(\alpha^t)$ to $\pi^{t}(\beta^{t})$}
}\label{alg:tree:phase}
\STATE  
$\pi^{t+1} \!\gets\! (\pi^{t} \setminus \{\pi^{t}(\alpha^t),\pi^{t}(\beta^t)\})\cup \{\pi^{t}(\beta^t)\cup \{\alpha^t\}\} \cup \{\, S \mid S~\mbox{is a maximal connected subset of}~\pi^{t}(\alpha^t)\!\setminus\!\{\alpha^t\}\,\}.$\label{alg:tree:ISdeviation}
\FOR{each $e \in L$} %\commentLuca{L_{\pi^t}(\alpha^t)} 
\IF{ $e \in L_{\pi^t}(\alpha^t) %\commentLuca{L_{\pi^t}(\alpha^t)} 
\cup \{(\alpha^t,\beta^t)\}$}
\STATE ${\ell^{t+1}}(e) \gets \alpha^t$ \label{alg:tree:label-update1}
\ELSE
%\FOR{each $e \notin L_{\pi^t}(\alpha^t) %\commentLuca{L_{\pi^t}(\alpha^t)}
%\cup \{(\alpha^t,\beta^t)\}$}
\STATE ${\ell^{t+1}}(e) \gets {\ell^{t}}(e)$ \label{alg:tree:label-update2}
\ENDIF
\ENDFOR
\STATE $t \gets t+1$
\ENDWHILE
\RETURN $\pi$
\end{algorithmic}
\end{algorithm}
\noindent Algorithm \ref{alg:is:tree} works as follows. 
At time step $t\geq 0$ player $\alpha^t$ performs a deviation from $\pi^{t}(\alpha^t)$ to $\pi^{t}(\beta^t)$ (see figure \ref{fig:tree:t-step}); $\pi^{t+1}$ denotes the partition obtained after  this deviation (line \ref{alg:tree:ISdeviation}).
As a consequence of Claim \ref{tree:claim1}, 
$(\alpha^t, \beta^t)$ is the only edge in $L_{\pi^{t+1}}(\alpha^t)$;   
%\commentLuca{$L_{\pi^{t+1}}(\alpha^t)$};
therefore we say that $\alpha^t$  \emph{builds} $(\alpha^t,\beta^t)$ and \emph{breaks} all the edges in $L_{\pi^{t}}(\alpha^t)$  %\commentLuca{$L_{\pi^{t}}(\alpha^t)$} 
at time $t$.
Moreover, as a consequence of Claim \ref{tree:claim1} and LAS preferences, $u_{\alpha^t}(\pi^{t+1}) =  v_{\alpha^t}(\beta^{t})$.

\begin{figure}
    \centering
\begin{subfigure}{0.2\textwidth}
    \centering
    \input{tree-fig-1}
    \caption{$\pi^t$}
    \label{fig:tree:t-step:A}
\end{subfigure}
\quad
\quad
\quad
\begin{subfigure}{0.2\textwidth}
    \centering
    \input{tree-fig-2}
    \caption{$\pi^{t+1}$}
    \label{fig:tree:t-step:B}
\end{subfigure}\caption{$t$-th steps of Algorithm \ref{alg:is:tree}.}
\label{fig:tree:t-step}
\end{figure}














Algorithm \ref{alg:is:tree} incorporates also a labeling scheme. 
At every time step $t\geq 0$, it assigns a label $\ell^t(e)$ to each edge $e = (i,j)  \in L$;
%\commentLuca{$e = (i,j) \in L$} 
this label gets  value in  $\{\bot, i, j\}$.
The label tracks which of the two endpoints of the edge made the most recent deviation in previous time steps, thereby determining the current status (built or broken) of the edge.
Namely, at time $t=0$  the label of each  edge  $e\in L$ is set  to $\bot$  (line \ref{alg:tree:label-init}), which means that none of the  endpoints of $e$  has   performed any deviation. 
At time $t+1\geq 1$ the labels of all the edges in $L_{\pi^t}(\alpha^t) \cup \{(\alpha^t,\beta^t)\}$ 
%incident to $\alpha^t$ 
are set to $\alpha^t$ 
%\commentLuca{not all the edges incident to $\alpha^t$, but only those in $L_{\pi^t}(\alpha^t) \cup \{(\alpha^t,\beta^t)\}$}
(line \ref{alg:tree:label-update1}), while the labels of all the remaining edges remain unchanged (line \ref{alg:tree:label-update2}). 
The labeling scheme satisfies the following property. 


  \begin{claim}\label{tree:claim:one-edge}
  For every $i\in N$ and $t\geq 0$, there exists at most one edge $e$ in $L_{\pi^t}(i)$ such that ${\ell^t(e)} = i$.
  \end{claim}
  \begin{proof}
  For $t=0$ the claim is trivial.  
  Hence,  let us assume $t\geq 1$.  
  	If $i$ has not performed any deviation in the previous time steps $1, 2, \ldots, t-1$ then no edge in $L_{\pi^t}(i)$ has label equal to $i$. 
  	Otherwise, let $t' < t$ be %\commentLaurent{initiated, because a deviation is somehow between two time steps} 
  the time step such that  $\alpha^{t'} = i$ and $\alpha^{t''} \neq i$, for every $t''$ such that  $t' < t'' < t$, i.e., $t'$ is the most recent time step in which $i$ has performed a deviation.  %\commentAngelo{I think this sufficient to}. 
   Then, 
   by Claim \ref{tree:claim1}, 
   %\commentLuca{by Claim \ref{tree:claim1}}, 
   $L_{\pi^{t'+1}}(i) = \{(i, \beta^{t'})\}$ and $\ell^{t'+1}((i, \beta^{t'})) = i$.
  	Since $i$ is not performing any deviation at any subsequent time step $t''$, $L_{\pi^{t''+1}}(i)$ will not contain any other edge with label $i$.  
  \end{proof}
  
%%%__OLD
% {\color{red}  
% The previous claim allows us to define the key concept of security value of a player.   
% The \emph{security value} $\kappa_i(\pi^t)$ of $i$ in $\pi^t$ is defined as follows: 
%  $\kappa_i(\pi^t) = v_i(j)$ if $e=(i,j) \in L_{\pi^t}(i)$ and $\ell^t(e)=i$, $\kappa_i(\pi^t) = 0$ otherwise. 
% Next, we will use the security value to bound the number of times a player $i$ can deviate by building an edge with a given neighbor $j$. Specifically, we will demonstrate that this occurs whenever the security value of a player drops to $0$.  
% First, let us examine how the security value of any player $i$ changes throughout the dynamics.
% Note that the security value of $i$ is influenced only by the deviations of $i$ and the deviations of the players in $N(i)$. Specifically, the security value of $i$ strictly increases after each deviation by $i$, while it strictly decreases (becoming equal to $0$) whenever a neighbor breaks the only edges incident to $i$ that are labeled $i$.
% This observation is formalized by the following claim. 
% \begin{claim}\label{tree:claim2-old}
% 	For every $i\in N$ and  $t\geq 0$ we have the  following:
% 	\begin{itemize}
% 		\item If $\alpha^t = i$  then $\kappa_i(\pi^{t}) < \kappa_i(\pi^{t+1})$ and $\kappa_i(\pi^{t+1}) = v_i(\beta^t)$; 
% 		\item If $\alpha^t \in N(i)$, $e=(\alpha^t,i) \in L_{\pi^{t}}(i)$ and  $\ell^t(e) = i$ then $\kappa_i(\pi^{t}) >  \kappa_i(\pi^{t+1}) = 0$;
% 		\item otherwise $\kappa_i(\pi^{t}) = \kappa_i(\pi^{t+1})$. 
% 	\end{itemize}
% \end{claim}
% }


Now, let us examine how the utility of any player $i$ changes throughout the dynamics given by an execution of Algorithm \ref{alg:is:tree}.
Note that the utility of $i$ is influenced only by the deviations of $i$ and the deviations of the players in $N(i)$. 
Moreover, note that, if  $v_i(j) = 0$, $i$ would never  perform a deviation in which she builds an edge with  $j$. 
Hence, the utility of $i$ strictly increases after each deviation by $i$, 
it may increase after a neighbour $j$ builds an edge with $i$ (it does not change if $v_i(j) = 0$),
it may decrease after a neighbor $j$ breaks an edge with $i$ (it does not change if $v_j(i) = 0$), while 
it strictly decreases after a neighbor $j$ breaks the edge with $i$ when its label is equal to $i$ (in fact, since the  edge has been previously built by $i$, it must hold that $v_i(j) > 0$). 
%\commentLaurent{In LAS preferences we have $v_i(j)>0 \Rightarrow (i,j) \in L$ but we don't have $v_i(j)>0 \Leftrightarrow (i,j) \in L$. For me, we don't necessarily have a strict increase after a neighbour builds an edge with $i$; same remark for strict decrease whenever a neighbor breaks an edge with $i$.}
%the only edges incident to $i$ that are labeled $i$.
This observation is formalized by the following claim. 
\begin{claim}\label{tree:claim2}
	For every $i\in N$ and  $t\geq 0$ we have the  following:
	\begin{itemize}
		\item If $\alpha^t = i$  then $u_i(\pi^{t}) < u_i(\pi^{t+1})$ and $u_i(\pi^{t+1}) = v_i(\beta^t)$;
        \item If $\alpha^t \in N(i)$, $e=(\alpha^t,i) \in {\overline L}_{\pi^{t}}(i)$ and $i  = \beta^t$ 
  then $u_i(\pi^{t}) \leq  u_i(\pi^{t+1})$; %\commentLaurent{For me it's $u_i(\pi^{t}) \leq  u_i(\pi^{t+1})$}
		\item If $\alpha^t \in N(i)$ and $e=(\alpha^t,i) \in L_{\pi^{t}}(i)$ %and  $\ell^t(e) = i$ 
  then $u_i(\pi^{t}) \geq  u_i(\pi^{t+1})$; 
  \item If $\alpha^t \in N(i)$, $e=(\alpha^t,i) \in L_{\pi^{t}}(i)$ and  $\ell^t(e) = i$ 
  then $u_i(\pi^{t}) >  u_i(\pi^{t+1})$;%\commentLaurent{Clarify whether $i \notin N(i)$ so that $i \neq \alpha^t$. For me it's $u_i(\pi^{t}) \geq  u_i(\pi^{t+1})$}
		\item otherwise $u_i(\pi^{t}) = u_i(\pi^{t+1})$. 
	\end{itemize}
\end{claim}



 
Next, we will bound the number of times a player $i$ can deviate by building an edge with a given neighbor $j$.
In order to do so, we need to introduce some notation. 
Let  $T_{Q}(i)$ denote the set of time  steps in which $i$ performs a deviation by building an edge connecting herself with any node in $Q\subseteq N(i)$. 
For $j\in N(i)$, we simplify the notation by writing $T_j(i)$ instead of $T_{\{j\}}(i)$.
Trivially, we have  $|T_{Q}(i)| = \sum_{j\in Q}|T_j(i)|$.
We denote by $T(i)$ the set of time steps in which $i$ performs a deviation, i.e., $T(i)  = T_{N(i)}(i)$. 
Since $i$ may also break edges with some neighbors during each deviation, for $j' \in N(i)$ and $Q
\subseteq N(i) \setminus \{j'\}$, we denote by $T^{j'}_{Q}(i)$ the set of time steps in which $i$ performs a deviation  by building an edge with any node in $Q$ while breaking the edge with $j'$ when its label is equal to $j'$.
For $j\in N(i)$, we simplify the notation by writing $T^{j'}_j(i)$ instead of $T^{j'}_{\{j\}}(i)$.
Trivially, we have  $|T^{j'}_{Q}(i)| = \sum_{j\in Q}|T^{j'}_j(i)|$.
We define $T^{j'}(i) = T_{N(i)\setminus \{j'\}}^{j'}(i)$, that is the set of time steps in which $i$ breaks the edge with $j' \in N(i)$ when its label is equal to $j'$. 
%Since, whenever $i$ is breaking the edge with $j'$, $i$ is also building an edge with some other neighbour in $N(i)\setminus \{j'\}$, we have  $T^{j'}(i) = T_{N(i)\setminus \{j'\}}^{j'}(i)$, and hence 
Also in this case we have $|T^{j'}(i)| = \sum_{j\in N(i)\setminus \{j'\}} |T^{j'}_{j}(i)|$.


\begin{figure}[h]
    \centering
    \input{tree-fig-sequence}
    \caption{Change of the utility of player $i$.}
    \label{fig:tree:sequence}
\end{figure}



% \begin{figure}[h]
% \caption{$t$-th steps of Algorithm \ref{alg:is:tree}.}
% 	\includegraphics[scale=0.13]{pic2.jpeg}
% \end{figure}


We are ready to show a bound on the number of times $i$ builds the  edge $(i,j)$.
\begin{claim}\label{tree:claim:join}
For every $i \in N$ and  $j\in N(i)$, 
\begin{align}
    |T_j(i)|
    &\leq 1 + \sum_{q \in N(i)} |T^{i}(q)|. \nonumber
\end{align}
\end{claim}
\begin{proof}
%%%___OLD
% {\color{red}
% 	From Claim \ref{tree:claim2} 
%  we can deduce that if there are two different time steps  in  which $i$ builds the edge with $j$ then there  must exist an intermediate time step in which the security value of $i$ has decreased.
% By Claim \ref{tree:claim2} the security value of $i$ decreases only when a neighbour breaks an edge with $i$ having label $i$. 
% This is fomalized as  follows.  
% 	Let $t, t'\in T_j(i)$, with $t < t'$.   
%     Then there must exist a time $\bar t$, with $t < \bar t < t'$, 
%     such that ${\bar t}  \in T^{i}(\alpha^{\bar t})$, i.e., $e= (i, \alpha^{\bar t}) \in L_{\pi^{\bar  t}}(i)$, $\ell^{\bar t}(e) = i$ and $\ell^{\bar t+1}(e) = \alpha^{\bar t} $.
% This implies that $i$ can build the edge with $j\in N(i)$ a number of times that is at most one plus the number of times that any player in $N(i)$ can break the edge with $i$.\\ 
% }
We consider the times steps depicted in figure  \ref{fig:tree:sequence}. 
Let $t, t'$ be two consecutive times steps in $T_j(i)$, i.e., $t<t'$  
%$t'' \not \in T_j(i)$ for every $t''$ with $t<t''<t'$. 
%$t+1 < t'$ 
%\commentAyumi{Sufficient to assume $t<t'$?}
and ${t''}  \notin T_j(i)$ for every $t < t'' < t'$. 
Notice that  $t' \neq t+1$. 
Since  $u_i(\pi^{t+1})  = u_i(\pi^{t'+1}) = v_i(j)$,  we  can deduce that there  must exist an intermediate time step in which the utility of $i$ has strictly decreased, and in  particular it must strictly decrease below $v_i(j)$. 
Let ${\bar t} + 1$ denote the first time step after $t$ such that $u_i(\pi^{{\bar t}+1})  <  v_i(j)$, i.e., 
$t +  1 < {\bar t}  + 1 \leq t'$ and, for every $t''$ such that $t + 1 \leq t'' \leq {\bar t}$, we have $u_i(\pi^{{t''}})  \geq  v_i(j)$.
%\commentAyumi{Check the following is still valid.}
By the  third and forth points of Claim \ref{tree:claim2} it must hold that at time $\bar t$ there must be some neighbour of $i$ that breaks  the  edge with $i$, i.e.,
$\alpha^{\bar t} \in N(i)$ and $(\alpha^{\bar t},i) \in L_{\pi^{\bar t}}(i)$.
We  want to show that there  must exists a  time  step $\tau$ such that $t+1 \leq \tau \leq \bar{t}$ and $\tau  \in T^{i}(\alpha^{\tau})$. 
%Notice that, by the forth point of Claim \ref{tree:claim2}, at time $\tau + 1$ ....
%such that  $\ell^{\tau}(e) = i$, and  hence  ${\bar t}  \in T^{i}(\alpha^{\bar t})$. %, that  is,  the  label of  $e=(\alpha^{\bar t},i)$  at time  $\bar t$ is $i$, i.e., $\ell^{\bar t}(e) = i$.  
Assume by contradiction that there is no such step $\tau$.
Then, by Claim \ref{tree:claim:one-edge}, in every time step $t''$ such that $t+1 \leq t'' \leq \bar{t} + 1$,  
there must always exist an edge in $L_{\pi^{t''}}(i)$ with label $i$. 
Let us denote by $e_{t''}$ the unique edge in $L_{\pi^{t''}}(i)$ with label $i$. 
Notice that $e_{t''}$ is either the edge $(i,j)$, built by $i$ at time $t$, or a new edge built by $i$ in a subsequent time step. 
Since, by the first point of Claim \ref{tree:claim2}, at every deviation of $i$ the utility of $i$ is strictly increasing, we must have that, if $e_{t''} = (i, j'')$, $v_i(j'') \geq v_i(j)$;
%it must hold that $e = (i,j) \in L_{\pi^{t''}}(i)$ and  $\ell^{t''}(e) = i$;
this implies $u_i(\pi^{t''}) \geq v_i(j'') \geq v_i(j)$ and hence $u_i(\pi^{\bar t  + 1}) \geq v_i(j)$. 
%\commentLuca{Assume by contradiction that there is no such step $\tau$, thus implying that $u_i(\pi^{\bar t+1}) \geq v_i(j)$.}
    % such that ${\bar t}  \in T^{i}(\alpha^{\bar t})$, i.e., $e= (i, \alpha^{\bar t}) \in L_{\pi^{\bar  t}}(i)$, $\ell^{\bar t}(e) = i$ and $\ell^{\bar t+1}(e) = \alpha^{\bar t} $.
% 	From Claim \ref{tree:claim2} 
%  we can deduce that if there are two different time steps  in  which $i$ builds the edge with $j$ then there  must exist an intermediate time step in which the security value of $i$ has decreased.
% By Claim \ref{tree:claim2} the security value of $i$ decreases only when a neighbour breaks an edge with $i$ having label $i$. 
% This is fomalized as  follows.  
% 	Let $t, t'\in T_j(i)$, with $t < t'$.   
%     Then there must exist a time $\bar t$, with $t < \bar t < t'$, 
%     such that ${\bar t}  \in T^{i}(\alpha^{\bar t})$, i.e., $e= (i, \alpha^{\bar t}) \in L_{\pi^{\bar  t}}(i)$, $\ell^{\bar t}(e) = i$ and $\ell^{\bar t+1}(e) = \alpha^{\bar t} $.
The existence of $\tau$ implies that $i$ can build the edge with $j\in N(i)$ a number of times that is at most one plus the number of times that any player in $N(i)$ can break the edge with $i$ when its label is equal to $i$.
\end{proof}




The previous claim implies the following key lemma. 
\begin{lemma}\label{tree:lemma:join}
For every $i\in N$ and $Q\subseteq N(i)$, 
\begin{align}
    |T_{Q}(i)|
    &\leq |Q|\left(1 + \sum_{q \in N(i)} |T^{i}(q)|\right). \nonumber
\end{align}  
\end{lemma}
%\commentLuca{the summation should be over $q \in N(i)$, right?}
%\commentAngelo{Yes. Fixed}


%Next, we bound $|T^{i}(j)|$ and $|T^{j'}_{j}(i)|$.  %the number of times $j$ breaks the edge with $i$.









\begin{claim}\label{tree:claim:break}
For every $i\in N$, with $|N(i)|\geq 2$, and $j,j'\in N(i)$, with $j\neq j'$,  
	\begin{align}
	|T^{j'}_j(i)|
    &\leq 1 + \sum_{q \in N(i)\setminus \{j'\}} |T^{i}(q)|.
\end{align}
%where $Q = N(j)\setminus\{i\}$.
\end{claim}
\begin{proof}
The proof of the claim is the proof of Claim \ref{tree:claim:join} with the additional observation that, due to the deviation of $i$ at time $t \in T^{j'}_j(i)$, we have $v_i(j') < v_i(j)$. 
This implies that before time $\tau$, $i$ never build an edge with $j'$ and hence $j'$ cannot  be the player breaking the edge labelled $i$ with $i$ at time $\tau$. 
%%%___OLD
% {\color{blue}
% Let $t, t'$, be two consecutive times steps in $T_j(i)$, i.e.,  $t < t'$ and, for every $t''$ with $t < t'' < t'$, ${t''}  \notin T_j(i)$.
% Applying the same  argument used in the proof of Claim \ref{tree:claim:join}, we  know there is a time step $\bar t$, i.e., $t < {\bar t} < t'$  in which the security value of $i$ has decreased.
% Specifically, let $\bar t$ denote the  first  time after $t$ when  this happens. 
% This implies that the  security  value of $i$ between $t$ and $\bar t$ cannot  decrease. 
% By Claim \ref{tree:claim2} the security value of $i$ decreases only when a neighbour breaks an edge with $i$ having label $i$. 
% Let  $p$ be the  neighbour  that breaks the  edge  with  $i$  having label $i$  at time $\bar t$.
% We distinguish two cases: $v_i(j') \leq  v_i(j)$ and $v_i(j') >  v_i(j)$. 
% In the first case, 
% since the  security  value of $i$ between $t$ and $\bar t$ cannot  decrease and since $v_i(j') \leq  v_i(j)$, we  have that $p\neq  j'$. 
% In the second case ....
% Hence the claim follows by applying the same argument  used in the  proof of  Claim \ref{tree:claim:join}. 
% }
\end{proof}

The previous claim implies the following key lemma. 
\begin{lemma}\label{tree:lemma:break}
For every $i\in N$, with $|N(i)|\geq 2$, $j'\in N(i)$ and $Q
 \subseteq N(i)\setminus \{j'\}$,
	\begin{align}
	|T^{j'}_{Q}(i)|
    &\leq |Q|\left(1 + \sum_{q \in N(i)\setminus \{j'\}} |T^{i}(q)|\right).\nonumber
\end{align}
%where $Q = N(j)\setminus\{i\}$.
\end{lemma}





% \begin{claim}
% \begin{align}
% 	|T^{i}(j)| \leq  |T_{Q}(j)|,\nonumber
% \end{align}
% where $Q = N(j)\setminus\{i\}$.
% \end{claim}
% \begin{proof}
% Every time $t\in T_{Q}(j)$ in which $j$ builds an  edge with a player in  $Q$, $j$ may break some  edge  with other neighbours.  
% Hence, let $J$ denote the number of times \commentLuca{it should be: let $J$ denote the set of time steps} in which $j$ breaks the edge with $i$, we have $J\subseteq T_{Q}(j)$. 
% The claim follows by observing that $T^{i}(j) \subseteq J$, in fact $T^{i}(j)$ coincides only with those time steps in which $j$ breaks the edge with  $i$ when this edge has label equal to  $j$.  
% \end{proof}

\iffalse
Next with give an alternative and simpler bound to $|T^{i}(j)|$.
\begin{claim}\label{tree:claim:break:simple}
For every $j\in N$ and $i\in N(j)$,  
	\begin{align}
	|T^{i}(j)|
    &\leq |T_{Q}(j)|.
\end{align}
where $Q = N(j)\setminus\{i\}$.
\end{claim}
\begin{proof}
Every time $t\in T_{Q}(j)$ in which $j$ builds an  edge with a player in  $Q$, $j$ may break some  edge  with other neighbours.  
Hence, let $J$ denote the number of times \commentLuca{it should be: let $J$ denote the set of time steps} in which $j$ breaks the edge with $i$, we have $J\subseteq T_{Q}(j)$. 
The claim follows by observing that $T^{i}(j) \subseteq J$, in fact $T^{i}(j)$ coincides only with those time steps in which $j$ breaks the edge with  $i$ when this edge has label equal to  $i$.  
\end{proof}
\fi



\bigskip

Now, let us consider a player $r$ and let $\hat G$ be the tree $(N,L)$ rooted in $r$.
Our goal is to bound the  number of deviations of $r$. 
We denote by $C_i$ the  set of children of $i$, by $D_i$  the  set of players in the  subtree of  $\hat G$ rooted in $i$ (including $i$) and by $p(i)$ the  parent of $i\neq r$.
Notice that  
$C_r = N(r)$, $D_r = N$, $C_i = N(i) \setminus \{p(i)\}$ for every $i\neq r$, and $C_i = \emptyset$ and $D_i = \{i\}$ for every leaf $i$. 
For every $i$, let $d_i$ be the maximum distance between $i$ and any leaf in $D_i$ ($d_i = 0$ for every leaf $i$). %\commentLaurent{maximum or minimum distance?}
For every path $\sigma_{j}^i=\langle j=q_0, q_1, \ldots, q_{k}=i\rangle$ such that $k\geq 0$ and   $q_{h+1}  = p({q_h})$ for every $h=0\ldots,k-1$, we define $m_j^i = \prod_{h=0}^k|C_{q_h}|$ (notice that $m^i_j=0$ for every leaf $j$). %\commentLuca{actually, if $i$ is a leaf, it holds $m_i^j=0$ for any $j$, right?}).
%\commentAngelo{Right! We can rewrite the  previous sentence as: notice that $m^i_j=0$ for every leaf $j$.}



\begin{lemma}\label{tree:moves:i}
For every $i\in N\setminus \{r\}$,
	\begin{align}
	|T^{p(i)}_{C_i}(i)| \leq   \sum_{j\in D_i} m_j^i.\nonumber
\end{align}
\end{lemma}
\begin{proof}
	Let $A_k = \{i\in N\setminus \{r\} : d_i \leq k\}$ for some  integer $k \in [0, d_r-1]$.
	We prove by induction on $k$ that the inequality  holds for every $i\in A_k$ and every $k$. 
	%The proof is by induction on $k$. \commentAyumi{Our proof}
	If $k=0$  then every $i\in A_k$ is a leaf which implies $C_i = \emptyset$ and $D_i=\{i\}$. Hence  both sides of the inequality are equal  to $0$. 
	Assume that the  claim is true for $A_k$, we prove the  claim for $A_{k+1}$.
	Let $i$ be any player in $A_{k+1}$.
 Since $C_i = N(i)\setminus \{p(i)\}$,
	from Lemma \ref{tree:lemma:break} we have 
	\begin{align}\label{tree:moves:step1}
    |T^{p(i)}_{C_i}(i)|
    &\leq |C_i|\big(1 + \sum_{q \in C_i
    %\commentLuca{N(i)??}
    } |T^{i}(q)|\big). 
\end{align}
Moreover, by definition, for every $q \in C_i$,
%Claim  \ref{tree:claim:break:simple}, %\commentLuca{for any $q \in C_i$,} 
\begin{align}\label{tree:moves:step2}
	|T^{i}(q)| = |T^i_{C_q}(q)|.
\end{align}
Finally, by inductive hypothesis, we have that for every $q\in C_i$ \begin{align}\label{tree:moves:step3}
	|T^i_{C_q}(q)| \leq \sum_{j\in D_q} m^q_j. 
\end{align}


Hence,  
	\begin{align}%\label{tree:moves:step4}
    |T^{p(i)}_{C_i}(i)|
    &\leq |C_i|\big(1 + \sum_{q \in C_i
    %\commentLuca{N(i)??}
    } \sum_{j\in D_q} m^q_j\big)\nonumber\\
    &= |C_i| + |C_i|\sum_{q \in C_i
    %\commentLuca{N(i)??}
    } \sum_{j\in D_q} m^q_j\nonumber\\
    &= m^i_i + \sum_{ q  \in C_i
    %\commentLuca{N(i)??}
    }  \sum_{j\in D_q} \left( |C_i| \cdot   m^q_j\right)\nonumber\\
    &= m^i_i + \sum_{ q  \in C_i
    %\commentLuca{N(i)??}
    } \sum_{j\in D_q} m^i_j\nonumber\\
    &=  
    \sum_{j\in D_i} m^i_j,\nonumber
\end{align}
where the first inequality follows by combining \eqref{tree:moves:step1},  \eqref{tree:moves:step2} and \eqref{tree:moves:step3}.   
\end{proof}







\begin{lemma}\label{tree:moves:r}
For the root $r$, we have
\begin{align}
	|T{(r)}| &\leq \sum_{j\in N} m^r_j.\nonumber
\end{align}
\end{lemma}


\begin{proof}
   	Since, $N(r) = C_r$, from Lemma \ref{tree:lemma:join} we have 
	\begin{align}%\label{tree:moves:r:step1}
   |T(r)| = |T_{C_r}(r)|  
   &\leq |C_r|\big(1 + \sum_{q \in C_r} |T^{r}(q)|\big). \nonumber
    \end{align}
    
Moreover, since $T^{r}(q) = T^{p(q)}_{C_q}(q)$, we can apply Lemma \ref{tree:moves:i} to the previous inequality and obtain, by exploiting the same arguments of Lemma \ref{tree:moves:i}, 
	\begin{align}%\label{tree:moves:r:step2}
   |T(r)|  
   &\leq |C_r|\big(1 + \sum_{q \in C_r}  \sum_{j\in D_q} m_j^q\big) =  \sum_{j\in D_r} m^r_j. \nonumber
    \end{align}
\end{proof}




The theorem follows from the arbitrary  choice of $r$. 
% If we apply the  previous lemma to the root $r$, we get
% \begin{align}
% 	|T{(r)}| \leq \sum_{j\in N(r)} m^r_j,  \nonumber
% \end{align}
% that is, the  total number of deviations of $r$ is bounded. 
% The theorem follows from the arbitrary  choice of $r$. 

==> stars_backup.tex <==
%\newpage
\section{Stars} \label{sec:stars}



\commentLaurent{Consider to put this section after trees, and/or some parts in the appendix. Or ignore stars for the conference version.}

This section deals with the special case where $(N,L)$ is a star. We will say that a coalition $S \subseteq N$ is {\em individually rational} if every player $i \in S$ weakly prefers $S$ to $\{i\}$. Moreover, a partition $\pi$ of $N$ is said to be {\em individually rational} if every $S \in \pi$ is individually rational. 
\commentLaurent{Maybe we could move the next sentence after Theorem 4.1. Actually, in Table 1, we say that Thm 4.1 gives the convergence in stars for IR prefs. In fact, this fact is a corollary of Theorem 4.1. With IR prefs, any state (including the initial one) is IR. }
It is worth noticing that starting from an individually rational state is a weaker requirement than imposing individually rational preferences.



\begin{theorem}\label{IS:stars}
 Suppose that $(N,L)$ is a star and the initial state is individually rational. 
Under general  
preferences, the IS dynamics converge in a number of steps polynomial in the number of players. \commentLaurent{...polynomial in $n$.}
\end{theorem}
\begin{proof}
Let $c$ denote the central player of the star. We refer to the coalition to which $c$ belongs as the \emph{central} coalition. 

We first show that if the initial state is individually rational, then individual rationality is preserved throughout the IS dynamics on a star. Indeed, suppose that $\pi$ is individually rational and there is a feasible deviation of player $j \in N$ to $T \in \pi \cup \{\emptyset\}$. Then, $T \neq \emptyset$ since $\pi$ is individually rational. Thus, either we have (i) $j=c$ and $T$ consists of a leaf of the graph $(N,L)$, or (ii) $j$ is a leaf of the graph and $T$ is the central coalition. In either case, the new partition $\pi'$ that results from the deviation of $i$ to $T$ (i.e., Line~\ref{line:ISdeviation} of Algorithm~\ref{alg:is:general}) is individually rational. 

Now, to show the \textcolor{red}{result,} %claim,  
observe that there are only two types of deviations, (i) and (ii), described above by the assumption that the initial state is individually rational. \textcolor{red}{Moreover, each of these deviations concerns the central player who is never worst off.} 
There are at most $n-1$ coalitions $\{j\}$ $(j \in N \setminus \{c\})$ to which the central player $c$ can deviate. \textcolor{red}{Furthermore}, there are at most $n-1$ players who can deviate to the \textcolor{red}{central coalition} %of the central player $c$ 
(no leaf player has an incentive to deviate from the central coalition once she joins it). Hence, the rank of the central coalition for $c$ can strictly increase at most $2n$ times during the dynamics, which implies a polynomial time convergence of the IS dynamics. 
\end{proof}

\commentLaurent{I have doubts on the $2n$ improvements in the previous proof, so I propose a new proof.} 
\commentLaurent{Let $c$ denote the central player of the star. We refer to the coalition to which $c$ belongs as the \emph{central} coalition. We first observe that if the initial state is IR, then individual rationality is preserved throughout the IS dynamics on a star. Indeed, suppose that $\pi$ is IR and there is a feasible deviation of player $j \in N$ to $T \in \pi \cup \{\emptyset\}$. Then, $T \neq \emptyset$ since $\pi$ is IR. Thus, either we have (i) $j=c$ and $T$ consists of a leaf of the graph $(N,L)$, or (ii) $j$ is a leaf of the graph and $T$ is the central coalition. In either case, the new partition $\pi'$ that results from the deviation of $i$ to $T$ (cf. Line~\ref{line:ISdeviation} of Algorithm~\ref{alg:is:general}) is IR. Now, to show the theorem,  observe that there are only two types of deviations, (i) and (ii), as described above. Each of them concerns the central player who is never worst off.  There are at most $n-1$ coalitions $\{j\}$, with  $j \in N \setminus \{c\}$, to which the central player $c$ can deviate. Moreover, there are at most $n-1$ players in $N \setminus \{c\}$ who can join the central coalition, and no such player benefits from leaving the central coalition. Hence, there are at most $n-1$ deviations of type (i), and at most $n-1$ deviations of type 
(ii) after a deviation of type (i). Hence, the IS dynamics converge after $\mathcal{O}(n^2)$ deviations.}


Note that without the assumption that the initial state is IR,  %individually rational, 
the IS dynamics may not converge on a star. 
\begin{example}\label{counterexample:star}
Consider a star with center $d$ and leaves $a,b,c$. 
Player $d$ is indifferent between all coalitions and the preferences of the other players are given as follows: 
%\commentLuca{I have added $\succ \{a,b,c,d\}$ at the end of all preference lists. In this way, this example also works for BEST responses.}
\begin{itemize}
\item $a: \{a,b,d\} \succ \{a\} \succ \{a,c,d\} \succ \{a,d\} \succ \{a,b,c,d\}$ 
\item $b: \{b,c,d\} \succ \{b\} \succ \{a,b,d\} \succ \{b,d\}\succ \{a,b,c,d\}$
\item $c: \{a,c,d\} \succ \{c\} \succ \{b,c,d\} \succ \{c,d\}\succ \{a,b,c,d\}$
\end{itemize}
The initial state is $\{\{a\},\{b,c,d\}\}$. Player $c$ forms her own coalition since $\{b,c,d\}$ is not individually rational for $c$, yielding $\{\{a\},\{b,d\},\{c\}\}$. 
Player $a$ then deviates to $\{b,d\}$, yielding $\{\{a,b,d\},\{c\}\}$. Player $b$ forms her own coalition, yielding $\{\{a,d\},\{c\},\{b\}\}$. 
Player $c$ then deviates to $\{a,d\}$, giving $\{\{a,c,d\},\{b\}\}$. Player $a$ forms her own coalition, yielding $\{\{c,d\},\{b\},\{a\}\}$. 
Player $b$ then deviates to $\{c,d\}$, yielding the initial state.
\end{example}

Moreover, %Note that 
even when the initial state is IR, 
% individually rational, 
the IS dynamics %Algorithm \ref{alg:is:general} 
can cycle in a %graph which is %almost a 
star %, i.e., a star 
with an extra %pendant 
node connected to a leaf (cf. Example \ref{ex:almoststar} in the appendix). 

\begin{comment}
\begin{example} \label{ex:almoststar}Consider the instance described in Figure \ref{fig:almost_star} where the preferences are: 
\begin{itemize}
\item $a: \{a,b\} \succ \{a,e\} \succ \{a,b,d\} \succ  \{a,d\}  \succ \{a\}$
\item $b: \{a,b,d\} \succ \{b,c\} \succ \{a,b\} \succ  \{b\}$
\item $c: \{b,c\} \succ \{c\}$
\item $d: \{a,b,d\} \succ \{a,d\} \succ \{d\}$
\item $e: \{a,e\} \succ \{e\}$

\end{itemize}
The initial state is $\{\{a,b\},\{c\},\{d\},\{e\} \}$. Player $b$ moves from $\{a,b\}$ to $\{c\}$ giving $\{\{a\},\{b,c\},\{d\},\{e\}\}$. Player $a$ moves from $\{a\}$ to $\{d\}$ giving $\{\{a,d\},\{b,c\},\{e\}\}$. Player $b$ moves from $\{b,c\}$ to $\{a,d\}$ giving $\{\{a,b,d\},\{c\},\{e\}\}$. Player $a$ moves from $\{a,b,d\}$ to $\{e\}$ giving $\{\{a,e\},\{b\},\{c\},\{d\}\}$. Player $a$ moves from $\{a,e\}$ to $\{b\}$ giving $\{\{a,b\},\{c\},\{d\},\{e\}\}$, which is the initial state.
%\commentLuca{This example works also for BEST responses. Moreover, in this example also the accepting players are always strictly improving.}
\end{example}


\begin{figure}
\caption{An ``almost'' star where the IS dynamics can cycle.} \label{fig:almost_star}
\begin{center}
\begin{tikzpicture}[node distance={10mm}, thick, main/.style = {draw, circle}] 
\node[main] (1) {$c$}; 
\node[main] (2) [above left of=1]  {$b$}; 
\node[main] (3) [below left of=2] {$a$}; 
\node[main] (4) [above left of=3] {$e$}; 
%\node[main] (5) [below of=3] {$d$}; 
\node[main] (5) [below left of=4] {$d$}; 



\draw[-] (1) -- (2);
\draw[-] (2) -- (3);
\draw[-] (4) -- (3);
\draw[-] (3) -- (5);

\end{tikzpicture} 
\end{center}

\end{figure}


\end{comment}


\commentLaurent{Write a new proof of convergence for IR prefs in stars, where the initial state is not necessarily IR. Update the table. Maybe place Thm 4.1 in the appendix.}
